Directed Cyclic Graph for Causal Discovery from Multivariate Functional Data

Discovering causal relationship using multivariate functional data has received a significant amount of attention very recently. In this article, we introduce a functional linear structural equation model for causal structure learning when the underlying graph involving the multivariate functions may have cycles. To enhance interpretability, our model involves a low-dimensional causal embedded space such that all the relevant causal information in the multivariate functional data is preserved in this lower-dimensional subspace. We prove that the proposed model is causally identifiable under standard assumptions that are often made in the causal discovery literature. To carry out inference of our model, we develop a fully Bayesian framework with suitable prior specifications and uncertainty quantification through posterior summaries. We illustrate the superior performance of our method over existing methods in terms of causal graph estimation through extensive simulation studies. We also demonstrate the proposed method using a brain EEG dataset.

==> Causal_Identifiability.tex <==
In this section, we shall show that the graph structure of the proposed FENCE model is identifiable for functional data measured discretely with random noises under several causal assumptions. We start by defining causal identifiability and state our assumptions.
\begin{definition}(\textit{Causal Identifiability})
Suppose $\bm{Y}$ is a $p$-variate random function and $\bm{X}$ is the observed noisy version of $\bm{Y}$ given by (\ref{eqn:2.2.6}). Assume $\bm{X}$ follows FENCE model $\mathcal{S} = (\mathcal{G}, \mathbb{P})$ where $\mathcal{G}$ is the underlying graph and $\mathbb{P}$ is the joint distribution of $\bm{X}$ over $\mathcal{G}$. We say that $\mathcal{S}$ is causally identifiable from $\bm{X}$ if there does not exist any other $\mathcal{S}^{*} = (\mathcal{G}^{*}, \mathbb{P}^{*})$ with $\mathcal{G}^{*} \neq \mathcal{G}$ such that the joint distribution $\mathbb{P^{*}}$ on $\bm{X}$ induced by $\mathcal{G}^{*}$ is equivalent to $\mathbb{P}$ induced by $\mathcal{G}$.

\end{definition}

In other words, for a causal graph to be identifiable, there must not exist any other graph such that the joint distributions induced by the two different graphs are equivalent. Next, we list and discuss a few assumptions to establish the causal identifiability of the proposed model.

\begin{assumption}(Causal Sufficiency)\label{ass1}
The model $\mathcal{S} = (\mathcal{G}, \mathbb{P})$ is causally sufficient, i.e., there are no unmeasured confounders.
\end{assumption}
Assuming no unmeasured confounders keeps the causal discovery task more manageable especially for cyclic graphs with purely observational data.

\begin{assumption}(Disjoint Cycles)\label{ass2}
The cycles in $\mathcal{G}$ are disjoint, i.e., no two cycles in the graph have two nodes that are common to both. 
\end{assumption}
Assuming disjoint cycles induces a natural topological ordering and forms a directed acyclic hypergraph-like structure within the DCG. The same assumption was made in \cite{Lacerda}.

\begin{assumption}(Stability)\label{ass3}
For the model $\mathcal{S}$, the moduli of the eigenvalues of the finite rank operator $\mathcal{B}$ are less than or equal to $1$, and none of the real eigenvalues are equal to $1$. 
\end{assumption}


According to \citealp{fisher}, the SEM in (\ref{eqn:2.2.4}) can be viewed as being in a state of equilibrium, where the finite rank operator $\mathcal{B}$ represents coefficients in a set of dynamical equations that describe a deterministic dynamical system observed over small time intervals as the time lag approaches zero. The eigenvalue conditions are deemed necessary and sufficient for the limiting behavior to hold, as argued by \citealp{fisher}. Such an assumption is widely adopted in e.g., econometrics, and \citealp{Lacerda} made this assumption as well. 


\begin{assumption}(Non-Gaussianity)\label{ass4}
The exogenous variables have independent mixture of Gaussian distributions.
i.e., $\epsilon_{jk} \overset{\text{ind}}{\sim} \sum_{m = 1}^{M_{jk}} \pi_{jkm} \text{N}(\mu_{jkm}, \tau_{jkm})$ with $M_{jk} \geq 2$.
\end{assumption}

The assumption of non-Gaussianity on the exogenous variables has been proven useful in causal discovery as it induces model identifiability in the linear SEM framework \citep{HP, shimizu06a, Lacerda, spirtes2016}. Mixture of Gaussian can approximate any continuous distribution arbitrarily well given a sufficiently large number of mixture components \citep{titterington_85, MCLA2000, rossi}. It is also easy to sample, which facilitates our posterior inference. 


\begin{assumption}\label{ass5}
(Non-causal dependency) We assume $\bm{\beta}(\bm{t}) = \bm{C}(\bm{t})\bm{\gamma}$, where $\bm{C}(\bm{t}) = diag(\bm{C}_{11}(\bm{t}_{1}), \dots, \bm{C}_{pp}(\bm{t}_{p}))$ and $\bm{\gamma}$ represent another exogenous component of the model. Here $\bm{C}_{jj}(\bm{t}_j)$ is a mixing matrix that mixes the independent entires in $\bm{\gamma}$ to generate temporal dependence within the $j$-th block. We assume $\gamma_{jk} \overset{\text{ind}}{\sim} \sum_{m = 1}^{M_{jk}} \pi_{jkm}' \text{N}(\mu_{jkm}', \tau_{jkm}')$ with $M_{jk}\geq 1$. 
\end{assumption}

Since the model assumes that all causal information in $\bm{Y}$ is preserved in the lower-dimensional space $\mathcal{D}_{j}$ and not in its orthogonal complement, it is apparent that while each $\bm{\beta}_{j}(\bm{t}_{j})$ within a block can have temporal dependence, it is independent of $\bm{\beta}_{\ell}(\bm{t}_{\ell})$ when $j\neq \ell$ and $j, \ell \in [p]$. 

For some basis $\{\phi_{jk}\}_{k=1}^{K_{j}}$ that spans the low-dimensional causal embedded space $\mathcal{D}_{j}$, $\alpha_{j}$ in (\ref{eqn:2.2.5}) can be further expanded by, $\alpha_{j}(t_{ju}) = \sum_{k = 1}^{K_{j}}\tilde{\alpha}_{jk}\phi_{jk}(t_{ju})$. Therefore (\ref{eqn:2.2.6}) can be written more compactly as 
\begin{equation}
    \bm{X} = \bm{\Phi}(\bm{t})\tilde{\bm{\alpha}} + \bm{\beta}(\bm{t}) + \bm{e},
    \label{eqn:2.2.7}
\end{equation}
where $\bm{\Phi}(\bm{t}) = \diag(\bm{\Phi}_{1}(\bm{t}_{1}), \dots, \bm{\Phi}_{p}(\bm{t}_{p}))$ with $\bm{\Phi}_{j}(\bm{t}_{j}) = (\phi_{jv}(t_{ju}))_{u=1, v=1}^{m_{j}, K_{j}}$.

\begin{assumption}\label{ass6}
(Sufficient sampling locations) The basis matrix $\bm{\Phi}(\bm{t})$ of size $\sum_{j=1}^{p}m_{j} \times \sum_{j=1}^{p}K_{j}$ has a full column rank. 
\end{assumption}

This assumption implies enough sampling locations, over which each random function $Y_j$ is observed, to capture all the causal information that $Y_j$ contains. 

Given these six assumptions, our main theorem establishes the causal identifiability of the proposed model.

\begin{theorem}\label{Th:1}
Under Assumptions \ref{ass1}--\ref{ass6}, $\mathcal{S} = (\mathcal{G}, \mathbb{P})$ is causally identifiable.
\end{theorem}


The proof essentially involves two steps as shown in Figure \ref{fig:1}. On the left-hand side (LHS) of the diagram, we depict the hypergraph-like structure that emerges when assuming the existence of disjoint cycles (Assumption \ref{ass2}), whereas, on the right-hand side (RHS), we offer a magnified view of the hypernodes (nodes containing simple directed cycle). Our approach to proving causal identifiability progresses from the LHS to the RHS. That is, we first prove the identifiability of the hypergraph-like structure depicted on the LHS of Figure \ref{fig:1}, and then we proceed to establish the identifiability of each simple directed cycle within every hypernode in the hypergraph. The detailed exposition of the proof can be found in Section \ref{section:proof} of the Supplementary Materials. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=10cm]{Identifiability-cut.pdf}
    \caption{Two important components of causal identifiability proof: (I) identifiability of directed acyclic hypergraph induced by disjoint cycles, and (II) identifiability of each disjoint cycle.}
    \label{fig:1}
\end{figure}





==> abstract.tex <==
\begin{abstract}
Discovering causal relationship using multivariate functional data has received a significant amount of attention very recently. In this article, we introduce a functional linear structural equation model for causal structure learning when the underlying graph involving the multivariate functions may have cycles. To enhance interpretability, our model involves a low-dimensional causal embedded space such that all the relevant causal information in the multivariate functional data is preserved in this lower-dimensional subspace. We prove that the proposed model is causally identifiable under standard assumptions that are often made in the causal discovery literature. To carry out inference of our model, we develop a fully Bayesian framework with suitable prior specifications and uncertainty quantification through posterior summaries. We illustrate the superior performance of our method over existing methods in terms of causal graph estimation through extensive simulation studies. We also demonstrate the proposed method using a brain EEG dataset. 
\end{abstract}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
